Deep Portrait Delighting

We present a deep neural network for removing undesirable shading features from an unconstrained portrait image, recovering the underlying texture. Our training scheme incorporates three regularization strategies: masked loss, to emphasize high-frequency shading features; soft-shadow loss, which improves sensitivity to subtle changes in lighting; and shading-offset estimation, to supervise separation of shading and texture. Our method demonstrates improved delighting quality and generalization when compared with the state-of-the-art. We further demonstrate how our delighting method can enhance the performance of light-sensitive computer vision tasks such as face relighting and semantic parsing, allowing them to handle extreme lighting conditions.

==> images/fileSources.tex <==
https://codepen.io/bbennett/pen/RwqmaP


(alternative) https://www.flickr.com/photos/debarshiray/31746084701/in/photolist-QnhYXX-Sfc8GA-2dQgpKG-S3RvXo-CkGuGv-y3SFGi-zwLrJw-YpxCfo-2a2gAv6-2emmNcc-2eRApph-MEff2t-2dHAkeQ-2dN781g-28kVmab-rvWp3s-FZhhFg-272swaK-25FxkDN-GoHyJC-2ffYy5w-xueYKk-PgiPYo-2c8shgq-2bQJtav-E1XhLD-Qc7fZw-R6LEeW-sBVMvP-2aiXwtm-2a1YQn8-DomNtv-2a5ijg5-2a18r97-24hxo9B-RfeZBJ-25GrxTe-QqpTiK-Q3nwct-2c8uoTj-2ajfDiE-2dPViEJ-2a18qt9-RfeZkm-PXhpqQ-S3Rxj1-2dafDqm-QUbYuY-LHV9Dm-28Ep6aW

(alternative) https://www.flickr.com/photos/byrdiegyrl/627721328/in/photolist-XteFw-atqDuH-2bfefzu-dNM3Xv-24zmmra-dxdEQr-2b8af6r-23bzTK7-HNDSNU-QGHkZm-ZUzjoe-S2hmtD-HMUfBw-RM2goJ-Ja8GRU-26HLx1z-23aRsSq-2ak4X2T-28kcjXo-S6AEDS-24eUPLH-25Wtx7M-GBoEm2-GgxzP8-24yAcwV-3JAjcy-29U58DK-jLhBVT-VoCXLW-24zm1jr-JGg6qq-PufV2L-4kPYFp-274JpHt-om4mhe-25WtTax-25SKcaq-24jszx4-pLAQ6s-Uz3Uhh-24yu8eP-RT5DRn-T9ofKz-hUQAb-24QCBAW-X5TSox-TGb5QP-24QG1SE-HmyDRs-bdFiXt/

(alternative) https://www.flickr.com/photos/gilmorec/5438187968/in/photolist-9hy8Pw-wGDt48-oeTm3M-Kcna5-7hPZLq-7CnAKQ-Y2QMqe-arH8Zu-qqeaBb-8AprmD-oy9TXX-PbFtUG-22WsTvP-9EG1U4-Cppzj-99yLbm-arEmNR-98UDrj-2ASmb-6B8vND-3Qv9wt-5nAXUH-Yc8TZj-tjnif4-4ypHJZ-9wLJf-bs6Z83-4h8cHL-74LtEk-287T1o8-8Dt8SR-gi5reo-HGenB-aPQbeM-dozMGe-ESrfvd-9gCc5-8YNXPu-ktwvFT-bUqYd-81AUmf-oy8cMi-SsmmsP-GxRsve-otyPnE-22Qzfs3-hHMnfr-9eFstg-hhfX-bBwLKi

(1) https://www.flickr.com/photos/debarshiray/50775661003/in/photolist-2kmSx26-5euwYL-BYxY5N-5aMy1z-5aLs3b-53pE8d-4U34kL-bVLGE8-wsxosQ-jZJ9Rk-5aMy9z-6U7kZi-wQk8en-2iSFYVi-RhwPb-dTMq9M-ciGSLU-2iJdne8-4ybH3-bDpbDA-5RXS1y-5LDktB-2majfzz-96d68T-7hpJMf-puTXxT-Goshv9-7U1pPA-2j8J9Rz-eKDCex-dFgEeT-aeuXPu-8Javwv-etFY6R-63CvA7-2kn7Ej9-4pWdpt-p3wTwz-tzjuGW-2j8FkWZ-dSwHfR-MMjgEA-HUjtmD-orEusb-9KCVXw-faaZWF-2iQdjbR-2iM68gr-9m5C5N-5hUp5p

(2) https://www.flickr.com/photos/28104476@N00/13717969614/ 

(3)http://farm4.static.flickr.com/3816/13913741533_77a1d697fb_b.jpg

(4) https://www.flickr.com/photos/53936799@N05/5882020795/

(5) https://www.flickr.com/photos/41087279@N00/33541878380/in/photolist-T6YTRW-27duW2S-26tTdz3-raN3J9-r7jRq5-pfanBx-sodRv5-JGFaLz-27kscps-tSuNhm-ZWjwJq-roE3TF-wDy7Kn-vewzY3-wUNQxG-M36AR8-2bnGXDX-rNnYao-27fBs8q-TzPn9g-sQMJ7d-wKaopu-24HFh4b-wGczT2-UN9Q1o-Qyf1zs-K2dqqr-9QcQnb-UUFJxK-22phSDK-275qC4k-rV2qvw-CGVair-BYUo4o-wuMQvK-GTMdNs-zT7GgK-DBScK9-JatVc8-EhGoen-2fDMRqs-26uTuZj-245PXs8-YzwJFm-QFdusT-JXkKUp-DXPx3k-Cq8uph-MiDbaG-Lm4zZr

(6) https://unsplash.com/photos/d0peGya6R5Y

(7) https://www.flickr.com/photos/35652152@N07/35952939643/in/photolist-27dVMMH-QnR1FW-TzF5nS-kSNMF-xy63es-q4rJcY-Rwsrii-2dFAN2n-23a5rng-25UYVZP-2321BHt-25QfUTq-ZwgX5C-9MgJYh-T6gJjG-sSKAYr-NBNEyN-noRBFq-MKxhEU-2epgHrd-8nRtv3-24sbcqG-274osFJ-FrcX9F-nkWqZY-3wU5Vi-EG4agb-HNQGSW-29E114m-Hvbyru-WM3dnH-Co7qjC-N29e16-jWKmNy-22CRjhs-dEQrD3-KFn6jQ-KAsBH-jR8m98-fE6hGx-25Hd67s-286aGCq-283b9UW-22e7Na4-ZGo2MS-FPdMDn-vLDLdC-BajZi7-TkbRxR-Jccrb4

(8) https://www.flickr.com/photos/draket/14061218393/in/album-72157605354563859/

(9) https://www.flickr.com/photos/hepp/14523923249/in/photolist-o8qUnP-oXWttV-27SPQ5w-yNAHxd-ykLmtt-27SPKiC-C8z2D6-wQJtiM-dJH5ym-fcmsrL-T9PGaL-K5BbqV-vTkQ8v-EK8PXZ-2hAWs8K-xVvBJH-2m8YJJF-2j9pzwW-C5qewm-j6yhuv-QotgLE-fCpCYH-xDNGBJ-qXjA6E-PFjuvf-HcGS5Q-PPzVgA-TvofQX-zUapsS-U2MX7w-Todffc-kR6QQT-U2MSrQ-UycwsQ-U2MVud-U2MVgs-Tkoi8L-2iVUtCQ-2iVUv6V-SgJgAu-SYgNV7-2m6a42c-TyfoFZ-Tyft96-2iWeL4d-SjnFKV-HyXqKW-7gNvvt-2iVX4A6-XHdR6S

(10) https://www.flickr.com/photos/noahtratley/40720414520/in/photolist-253jLyq-27peUjN-FMSG2t-D3xVKn-LeWTbN-Y45NJS-27Q9LvP-2daxN4G-2bBcwKH-24BWQNh-GiUPW2-Ze4RXS-Qxx4v2-24tbqnF-R1eKeK-DKDzm9-UN3jYr-2a3vE3G-264hphb-RHdsMn-ZHj8Fq-GT5BdF-QtfaaB-2b4zwdT-23akYZd-Mp68K9-HjW88F-LF3WvK-JUzMEV-r6dfuA-27QQuPi-2cVQv7A-E1JnG6-Kyio2h-2btLRNz-RACjVT-KcQUL3-va9KSb-rb3egJ-RACjEx-yghWbh-KwkTrv-H49CjK-282QcX5-KemJT7-GgTTVy-vPxYEq-Dz5ExZ-zfF3Gc-2atWhou

(11) https://www.flickr.com/photos/scotgovrural/40262885703/in/photolist-24kTPbx-DJ8V7h-25wpohN-29y8eTQ-JrZwDH-ZrkAqe-YefcxA-Ctq8PY-GVEAaD-2dSow7a-YQeqLA-23rSuSk-2aXtY7m-28MGVpa-Eidda9-ZQvGyj-25Xtpfs-WwuoeW-2eTFdnV-26XCDD3-29CRp6i-24maqK9-2aC62Ys-MpeStZ-RBkUxU-26VYESq-Zt293P-28xwjmY-Sap6Yv-Y9bcqd-26VYb6Y-21r3wpa-24cFcpf-21wWukX-27jbaWL-27ZcfNH-C8DMKG-JvHy7a-Z4oHgu-HYdgPz-LAphgH-YDobCx-Mv4C3j-28x488Q-YvYxVc-ZbWhfJ-2cuaLnS-Lh2c6K-MZiABY-244cU8v



